Surface rotation and photometric activity for Kepler targets. II. G and F main-sequence stars, and cool subgiant stars

Dark magnetic spots crossing the stellar disc lead to quasi-periodic brightness variations, which allow us to constrain stellar surface rotation and photometric activity. The current work is the second of this series (Santos et al. 2019; Paper I), where we analyze the Kepler long-cadence data of 132,921 main-sequence F and G stars and late subgiant stars. Rotation-period candidates are obtained by combining wavelet analysis with autocorrelation function. Reliable rotation periods are then selected via a machine learning (ML) algorithm (Breton et al. 2021), automatic selection, and complementary visual inspection. The ML training data set comprises 26,521 main-sequence K and M stars from Paper I. To supplement the training, we analyze in the same way as Paper I, i.e. automatic selection and visual inspection, 34,100 additional stars. We finally provide rotation periods Prot and associated photometric activity proxy Sph for 39,592 targets. Hotter stars are generally faster rotators than cooler stars. For main-sequence G stars, Sph spans a wider range of values with increasing effective temperature, while F stars tend to have smaller Sph values in comparison with cooler stars. Overall for G stars, fast rotators are photometrically more active than slow rotators, with Sph saturating at short periods. The combined outcome of the two papers accounts for average Prot and Sph values for 55,232 main-sequence and subgiant FGKM stars (out of 159,442 targets), with 24,182 new Prot detections in comparison with McQuillan et al. (2014). The upper edge of the Prot distribution is located at longer Prot than found previously.

==> tab1.tex <==
\begin{rotatetable*}
\begin{deluxetable*}{ccccccccccccc}
\tablecaption{[Sample of the full table] Stellar properties for stars with successfully recovered rotation period. \teff, \logg, and mass from B20 when available, otherwise DR25 \citep{Mathur2017,Berger2020}. The rotation period and photometric activity estimates are obtained in this work. CP/CB candidate flag: (1) Type 1 CP/CB candidate. Subsample: (1) targets in subsample I; (2) targets in subsample II; and (3) targets in subsample III. Binary flag: (0) single stars in \citet{Berger2018} or in \citet{Simonian2019}; (1) targets flagged as binary candidates in \citet{Berger2018}; (2) targets flagged as binary candidates in \citet{Simonian2019} according to their inclusive threshold; (3) binary canidates in both \citet{Berger2018} and \citet{Simonian2019}. KOI flag: (0) confirmed planet hosts; (1) candidate planet hosts; (2) and false-positives. Source for stellar properties: (0) B20; (1) DR25. \label{tab1}}
\tablewidth{\hsize}
\tabletypesize{\fontsize{8.5}{10.}\selectfont}
%\movetabledown=-5in
\tablehead{
\colhead{KIC\vspace{-0.02cm}} & \colhead{Kp\vspace{-0.02cm}} & \colhead{Q\vspace{-0.02cm}} & \colhead{\teff\vspace{-0.02cm}} & \colhead{\logg\vspace{-0.02cm}} & \colhead{Mass\vspace{-0.02cm}} & \colhead{\prot\vspace{-0.02cm}} & \colhead{\sph\vspace{-0.02cm}} & \colhead{CP/CB\vspace{-0.02cm}} & \colhead{subsample\vspace{-0.02cm}} & \colhead{binary \vspace{-0.02cm}} & \colhead{KOI\vspace{-0.02cm}} & source\\
 &  &  & \colhead{(K)} & \colhead{(dex)} & \colhead{($M_\odot$)} & \colhead{(days)} & \colhead{(ppm)} & \colhead{cand.} & & \colhead{flag} & 
} 
\startdata
757099 & 13.152 & 1-17 & $5364.9^{+102.7}_{-84.9}$  & $4.318^{+0.037}_{-0.029}$ & $0.873^{+0.054}_{-0.039}$ & $0.38\pm0.02$  & $15463.8\pm1668.0$ & 1  & 1 &  0 & -- & 0\\
757450 & 15.264 & 1-17 & $5301.2^{+111.0}_{-103.1}$ & $4.432^{+0.045}_{-0.044}$ & $0.914^{+0.062}_{-0.057}$ & $19.11\pm1.50$ & $3756.4\pm118.7$   & -- & 1 &  0 & 0 & 0\\
891916 & 14.799 & 1-17 & $5650.8^{+131.9}_{-137.7}$ & $4.132^{+0.224}_{-0.254}$ & $1.008^{+0.164}_{-0.112}$ & $5.45\pm0.42$  & $3409.6\pm199.2$   & -- & 1 &  -- & -- & 0\\
892195 & 13.757 & 1-17 & $5333.4^{+101.3}_{-84.2}$  & $4.372^{+0.039}_{-0.029}$ & $0.862^{+0.057}_{-0.040}$ & $21.78\pm2.90$ &  $212.9\pm4.7$     & -- & 1 &  0 & -- & 0\\
892713 & 12.082 & 0-17 & $6238.9^{+123.4}_{-129.8}$ & $3.548^{+0.066}_{-0.037}$ & $1.731^{+0.219}_{-0.087}$ & $5.78\pm0.76$  &  $390.4\pm11.9$    & -- & 1 &  0 & -- & 0\\
893209 & 13.087 & 1-17 & $6051.4^{+110.0}_{-107.2}$ & $4.031^{+0.037}_{-0.053}$ & $1.263^{+0.071}_{-0.117}$ & $4.58\pm0.44$  &  $605.3\pm20.8$    & -- & 1 &  0 & -- & 0\\
893286 & 15.345 & 1-17 & $5297.1^{+103.4}_{-98.5}$  & $4.522^{+0.034}_{-0.044}$ & $0.853^{+0.047}_{-0.057}$ & $24.54\pm2.23$ & $1079.3\pm36.1$    & -- & 1 &  0 & -- & 0\\
893383 & 14.281 & 1-17 & $5680.9^{+105.1}_{-102.2}$ & $4.526^{+0.020}_{-0.031}$ & $0.912^{+0.036}_{-0.051}$ & $21.19\pm2.58$ &  $967.2\pm31.5$    & -- & 1 &  0 & -- & 0\\
893505 & 14.248 & 3-16 & $5920.4^{+123.8}_{-118.5}$ & $3.896^{+0.058}_{-0.044}$ & $1.239^{+0.143}_{-0.075}$ & $10.81\pm0.81$ &  $617.9\pm34.1$    & -- & 1 &  0 & -- & 0\\
893507 & 12.517 & 2-16 & $5447.0^{+121.8}_{-124.5}$ & $3.580^{+0.028}_{-0.039}$ & $1.510^{+0.075}_{-0.095}$ & $10.98\pm0.86$ & $7019.0\pm293.3$   & -- & 1 &  0 & -- & 0\\
893559 & 15.818 & 1-17 & $5095.3^{+95.2}_{-88.7}$   & $4.546^{+0.033}_{-0.041}$ & $0.808^{+0.044}_{-0.049}$ & $14.69\pm1.06$ & $2183.0\pm 87.9$ & -- & 1 & 0 & -- & 0\\
893676 & 15.310 & 1-17 & $5260.0^{+81.3}_{-72.5}$   & $4.211^{+0.037}_{-0.037}$ & $0.881^{+0.031}_{-0.024}$ & $24.37\pm2.73$ & $1227.7\pm 39.9$ & -- & 1 & 1 & -- & 0\\
1025986 & 10.150& 0-17 & $5662.1^{+101.7}_{-100.1}$ & $4.425^{+0.039}_{-0.042}$ & $0.912^{+0.066}_{-0.064}$ &  $9.68\pm0.73$  & $5940.1\pm245.0$ & -- & 1 & 0 & 1 & 0\\
1026838 & 13.897& 1-17 & $6056.9^{+101.3}_{-101.9}$ & $4.399^{+0.020}_{-0.030}$ & $1.133^{+0.041}_{-0.056}$ & $15.56\pm1.85$ & $ 361.9\pm 16.1$ & -- & 1 & 0 & -- & 0\\
1027536 & 12.886& 0-17 & $5944.4^{+117.2}_{-105.9}$ & $4.304^{+0.033}_{-0.038}$ & $1.139^{+0.066}_{-0.069}$ & $16.35\pm4.43$ & $  74.4\pm  5.0$ & -- & 1 & 0 & -- & 0\\
\enddata
\end{deluxetable*}
\end{rotatetable*}


==> tab2.tex <==
\begin{rotatetable*}
\begin{deluxetable*}{ccccccccccc}
\tablecaption{[Sample of the full table] Stellar properties for stars without rotation-period estimate. Same as in Table~\ref{tab1}, with exception of the no \prot\ flag which indicates the type target: (0) no rotational modulation; (1) possible rotational modulation; (2) misclassified red-giant star; (3) known eclipsing binary; (4) known RR Lyrae; (5) known $\delta$ Scuti, $\gamma$ Doradus, or hybrids; (6) photometric pollution in KEPSEISMIC and PDC-MAP time-series; (7) photometric pollution in KEPSEISMIC time-series; (8) multiple signals; (9) Type 2 CP/CB candidate; (10) Type~3 CP/CB candidate; (11) Type~4 CP/CB candidates.\label{tab2}}
\tablewidth{\hsize} 
\tabletypesize{\fontsize{8.5}{10.}\selectfont}
%\tabletypesize{\fontsize{8}{10.}\selectfont}
\tablehead{
\colhead{KIC\vspace{-0.02cm}} & \colhead{Kp\vspace{-0.02cm}} & \colhead{Q\vspace{-0.02cm}} & \colhead{\teff\vspace{-0.02cm}} & \colhead{\logg\vspace{-0.02cm}} & \colhead{Mass\vspace{-0.02cm}} & \colhead{no \prot\vspace{-0.02cm}} & \colhead{subsample} & \colhead{binary \vspace{-0.02cm}} & \colhead{KOI\vspace{-0.02cm}} & source\\
 &  &  & \colhead{(K)} & \colhead{(dex)} & \colhead{($M_\odot$)} & \colhead{flag} & & \colhead{flag} & &
} 
\startdata
757280 & 11.901 & 0-17 & $6856.8^{+144.4}_{-139.9}$ & $3.834^{+0.033}_{-0.032}$ & $1.715^{+0.086}_{-0.089}$ & 8 & 2 & 0 & -- & 0\\
891901 & 13.306 & 0-17 & $6350.6^{+130.8}_{-131.7}$ & $3.958^{+0.098}_{-0.090}$ & $1.411^{+0.125}_{-0.119}$ & 8 & 1 & -- & -- & 0\\
892203 & 13.575 & 0-17 & $5712.8^{+108.3}_{-105.3}$ & $4.386^{+0.042}_{-0.044}$ & $0.967^{+0.073}_{-0.074}$ & --& 1 & 0 & -- & 0\\
892667 & 13.137 & 1-17 & $6704.9^{+148.8}_{-128.8}$ & $3.950^{+0.034}_{-0.036}$ & $1.548^{+0.081}_{-0.087}$ & 5 & 2 & 0 & -- & 0\\
892675 & 13.475 & 1-17 & $5929.4^{+108.9}_{-108.1}$ & $4.385^{+0.035}_{-0.043}$ & $1.038^{+0.066}_{-0.076}$ & 0 & 1 & 0 & -- & 0\\
892678 & 12.176 & 0-17 & $5890.4^{+121.6}_{-114.9}$ & $3.574^{+0.030}_{-0.030}$ & $1.584^{+0.071}_{-0.062}$ & --& 1 & 0 & -- & 0 \\
892828 & 13.195 & 0-17 & $6464.3^{+137.7}_{-128.9}$ & $4.034^{+0.032}_{-0.034}$ & $1.398^{+0.071}_{-0.069}$ & 5 & 1 & 0 & -- & 0 \\
892911 & 15.648 & 2-17 & $5782.1^{+116.5}_{-112.6}$ & $4.295^{+0.062}_{-0.062}$ & $1.001^{+0.077}_{-0.077}$ & --& 1 & 0 & -- & 0 \\
892946 & 15.882 & 4-17 & $5993.8^{+122.3}_{-119.6}$ & $3.859^{+0.113}_{-0.113}$ & $1.317^{+0.157}_{-0.120}$ & 0 & 1 & 0 & -- & 0 \\
892977 & 13.759 & 1-17 & $6072.9^{+116.6}_{-116.6}$ & $3.937^{+0.044}_{-0.048}$ & $1.299^{+0.126}_{-0.090}$ & --& 1 & 0 & -- & 0 \\
892986 & 15.974 & 4-17 & $5770.8^{+115.8}_{-114.4}$ & $4.093^{+0.083}_{-0.090}$ & $1.068^{+0.101}_{-0.086}$ & 0 & 1 & 0 & -- & 0 \\
893004 & 13.957 & 1-17 & $6107.3^{+129.4}_{-115.7}$ & $4.171^{+0.044}_{-0.040}$ & $1.189^{+0.067}_{-0.091}$ & --& 1 & 0 & -- & 0 \\
893165 & 13.340 & 0-17 & $5989.1^{+115.7}_{-102.5}$ & $4.154^{+0.038}_{-0.042}$ & $1.152^{+0.073}_{-0.092}$ & 1 & 1 & 0 & -- & 0 \\
893234 & 13.195 & 1-17 & $6558.2^{+128.9}_{-141.2}$ & $4.112^{+0.033}_{-0.032}$ & $1.371^{+0.068}_{-0.060}$ & 5 & 1 & 0 & -- & 0 \\
893468 & 15.439 & 1-17 & $6016.0^{+112.0}_{-110.0}$ & $4.368^{+0.048}_{-0.058}$ & $1.067^{+0.067}_{-0.075}$ & 0 & 1 & 0 & -- & 0 \\
\enddata
\end{deluxetable*}
\end{rotatetable*}
